emg2pose: A Large and Diverse Benchmark for Surface Electromyographic Hand Pose Estimation

Hands are the primary means through which humans interact with the world. Reliable and always-available hand pose inference could yield new and intuitive control schemes for human-computer interactions, particularly in virtual and augmented reality. Computer vision is effective but requires one or multiple cameras and can struggle with occlusions, limited field of view, and poor lighting. Wearable wrist-based surface electromyography (sEMG) presents a promising alternative as an always-available modality sensing muscle activities that drive hand motion. However, sEMG signals are strongly dependent on user anatomy and sensor placement, and existing sEMG models have required hundreds of users and device placements to effectively generalize. To facilitate progress on sEMG pose inference, we introduce the emg2pose benchmark, the largest publicly available dataset of high-quality hand pose labels and wrist sEMG recordings. emg2pose contains 2kHz, 16 channel sEMG and pose labels from a 26-camera motion capture rig for 193 users, 370 hours, and 29 stages with diverse gestures - a scale comparable to vision-based hand pose datasets. We provide competitive baselines and challenging tasks evaluating real-world generalization scenarios: held-out users, sensor placements, and stages. emg2pose provides the machine learning community a platform for exploring complex generalization problems, holding potential to significantly enhance the development of sEMG-based human-computer interactions.

==> sections/emg_background.tex <==
\section{Surface Electromyography Sensing}
\label{sec: EMG background}

% \jm{@SS Your points about sEMG sensing in general here are good. We should have a paragraph in the introduction that mentions them explicitly. This paragraph also mixes in more specific comments about the EMG2Pose problem and belief state estimation and blind source separation and generalization. I think it would be better to separate the general features of sEMG from the specific aspects of the emg2pose problem. Note that also this background on challenges with emg2pose appear are mentioned in the previous section, but this background is logically prior, so I would reorganize a bit.}
% Surface electromyography (sEMG) measures electrical potentials generated by muscles close to the sensors \citep{stashuk2001emg}. Specifically, sEMG detects the motor neuron impulses that lead to the muscle fiber contractions and expansions that drive motion \citep{merletti2016surface}. Hand pose estimation from wrist-based sEMG is non-trivial introducing several challenges: (i) sEMG encodes muscle activity that drives joint accelerations, rather than pose directly. As such, sEMG as an observation space for pose inference is partially observable, obfuscating learning and presenting the challenge of belief state estimation \citep{monahan1982state,spaan2012partially,gu2021efficiently}.\rw{i think these ideas can be more clearly expressed w/out reference to belief state estimation or partial observability} (ii) The human hand is highly articulated, with $21$ degrees of freedom\ss{check this}, resulting in a large search space of comparable complexity to full body estimation. This hinders learning efficacy and generalization in low-data regimes, as well as belief state estimation \citep{thrun2002probabilistic,bishop2006pattern}. (iii) In the hand and forearm, there exists in the order of a thousand \ss{check this} motor neurons whose activities are superimposed in a complex non-linear manner, before being sensed\rw{remove 'before being sensed'}. This makes it particularly difficult to decouple individual joint and finger movements from the observations, and is itself a blind source separation problem with partial observability \citep{cardoso1996equivariant, hyvarinen2016unsupervised, halva2021disentangling}. (iv) Each user has a different anatomy, with distinct number of hand and forearm muscles \rw{most people have the same number of muscles; this is really an edge case}, muscle tendon attachments and locations relative to the sensors. 
% % In addition, each user has differing motor neuron impulse signatures \citep{todo}. 
% Furthermore, during activity, muscle locations vary. Altogether, these sources of variation not only make learning a generalized model across users difficult, but also zero-shot generalization to new users, in new contexts, particularly challenging \citep{saponas2008demonstrating,ctrl2024generic}. (v) Device placement and orientation heavily influences the location of muscles relative to the sensors, and therefore the observations. Wrist-based sEMG wearables will be taken on and off frequently, making this problem particularly important to address. Invariance to device placement is an open problem \citep{sussillo2016making, zia2018multiday}. Despite the above challenges, prior works have demonstrated huge potential in the personalized or single user pose inference settings \citep{liu2021neuropose,simpetru2022accurate}. 

There exist several sEMG platforms\rw{", which vary from low=density ... to high-density ..."} from low-density of sensors \citep{rawat2016evaluating} \ss{struggling to get an actual citation to an official web link to MYO armband website.} to high-density \citep{amma2015advancing} \jm{Can you make sure there are clear topic sentences for each of these paragraphs? Here the focus is a bit broader than just band density}\ss{@jesse - does your comment still apply given the restructuring?}\jm{can you move material about sEMG and generalization to the intro and the technical details to the appendix}. \rw{sentence here pointing out limitations of existing devices, then the next sentences introduces our device as a solution to these problems} Recently, \citet{ctrl2024generic} demonstrated the potential of the medium-density sEMG-RD wrist band for both generalized and personalized discrete gesture classification tasks across a populous of $6400$ participants, the largest study to date. Given this, we also use the sEMG-RD platform for data collection.\rw{i think we can remove the 'given this' sentence} \ss{Mostly copied from emg2qwerty - is this ok?} \rw{new paragraph?} In short, sEMG-RD consists of $16$ differential electrode pairs utilizing dry goal-plated electrodes. Signals are sampled at 2~kHz with a bit depth of 12 bits, with a maximum signal amplitude of 6.6~mV. Measurements are bandpass filtered with -3~dB cutoffs at 20~Hz and 850~Hz before digitization. The 16 electrodes are arranged on a rigid ribbon, leaving a gap between electrodes 0 and 15 on the ulnar side of the wrist close to the ulnar styloid. Identical bands are worn on the left and right hands, with the same electrode indices aligning with the same anatomical features, but the polarity of the differential sensing being reversed. The band is tightened with an elastic strap and the size of the gap depends on the subject's wrist size and tightness. The band is manufactured in three different sizes to account for large changes in wrist size and the electrodes themselves are spring-loaded to further adjust across small variations in wrist sizes. In contrast, the commonly used low-density MYO band \citep{rawat2016evaluating} only streams data at $200$Hz, across $8$ channels and at $8$-bits \ss{@Rick - can you confirm that only our band uses differential sensing? In which case I'll add that line.}.\rw{i'll look into it; thanks for adding this sentence. i think these points can be moved to the first paragraph. see my comments above}\ep{This paragraph feels very thin to cover an entire section. I would suggest moving the description of the band to section 4 and the references to the multi-user paper to section 3.}
